Depth Sensing Beyond LiDAR Range

Depth sensing is a critical component of autonomous driving technologies, but today's LiDAR- or stereo camera-based solutions have limited range. We seek to increase the maximum range of self-driving vehicles' depth perception modules for the sake of better safety. To that end, we propose a novel three-camera system that utilizes small field of view cameras. Our system, along with our novel algorithm for computing metric depth, does not require full pre-calibration and can output dense depth maps with practically acceptable accuracy for scenes and objects at long distances not well covered by most commercial LiDARs.

==> 060_limitations.tex <==
\section{Limitations}
Although we've tried our best to validate our algorithms, experiments in real-world driving scenarios have not been performed thoroughly because of resource and facility constraints.
In fact, part of our goal with this work was to devise a suitable approach in order to gain confidence in a vehicle-based deployment---a next step is to build a hardware system for autonomous vehicles, and test it on the road.
 
 



